Training Constrained Deconvolutional Networks for Road Scene Semantic Segmentation

In this work we investigate the problem of road scene semantic segmentation using Deconvolutional Networks (DNs). Several constraints limit the practical performance of DNs in this context: firstly, the paucity of existing pixel-wise labelled training data, and secondly, the memory constraints of embedded hardware, which rule out the practical use of state-of-the-art DN architectures such as fully convolutional networks (FCN). To address the first constraint, we introduce a Multi-Domain Road Scene Semantic Segmentation (MDRS3) dataset, aggregating data from six existing densely and sparsely labelled datasets for training our models, and two existing, separate datasets for testing their generalisation performance. We show that, while MDRS3 offers a greater volume and variety of data, end-to-end training of a memory efficient DN does not yield satisfactory performance. We propose a new training strategy to overcome this, based on (i) the creation of a best-possible source network (S-Net) from the aggregated data, ignoring time and memory constraints; and (ii) the transfer of knowledge from S-Net to the memory-efficient target network (T-Net). We evaluate different techniques for S-Net creation and T-Net transferral, and demonstrate that training a constrained deconvolutional network in this manner can unlock better performance than existing training approaches. Specifically, we show that a target network can be trained to achieve improved accuracy versus an FCN despite using less than 1\% of the memory. We believe that our approach can be useful beyond automotive scenarios where labelled data is similarly scarce or fragmented and where practical constraints exist on the desired model size. We make available our network models and aggregated multi-domain dataset for reproducibility.

==> srcs/supmat.tex <==
\appendix{\huge Supplementary Material}

\section{Dataset: Refinement of bounding box annotations.}

For those datasets where annotations are provided in the form of bounding boxes, we refine these to pixel-wise 
annotations suitable for DN training by adopting a similar technique to~\cite{Papandreu15iccv}: %for obtaining semantic labels from bounding box annotations.
we use the GrabCut algorithm~\cite{Rother04sg} to segment the foreground object pixels from the background. We constrain the central area of the bounding box ($\alpha \%$ of pixels within the box) to be foreground, while the pixels 
outside the bounding box of the object of interest and the pixels inside the remaining bounding boxes of the other annotated objects in the 
image are constrained as background. \SI{what is alpha?}

We perform additional refinement on the CBCL dataset, which consists of 3,547 images with polygonal bounding boxes for 9 object categories (car, 
pedestrian, bicycle, building, tree, sky, road, sidewalk and store). It was created for object detection and contains missing 
labelled objects, ambiguous labelling situations and objects that are not tightly bound within the polygon annotations. We re-labelled and 
extended the categories for 584 of the images containing dense pixel-wise annotations and produced semi-supervised annotations for the 
remaining 2,963 images by applying a CRF classifier~\cite{Ladicky10eccv} combined with the polygon-based ground truth.

\subsection{Results}

Images are initially normalized using spatial contrast normalization, independently applied to each channel $f$ as $\bar{X}_{i,j,f} = X_{i,j,f} / (1 + \alpha  \frac{1}{k^2}\sum_{j'=0}^{k-1}{\sum_{i'=0}^{k-1}{x^2_{i+i',j+j',f}}})^\beta$. Here $k=7$ stands for the kernel size and $\alpha = 1, \ \beta=0.5$.

\begin{table*}[]
	\centering
	\caption{Semantic segmentation quantitative results on the testing dataset, training with the Sparse domain.}
	\vspace{-3mm}
	%\resizebox{\textwidth}{!}{%
		\scriptsize
		\tabcolsep=0.06cm
		\begin{tabular}{@{}lcccccccc@{}}
			\toprule
			Method    & other & pole & car & sign & pedestrian & cyclist & \textbf{per-class} & \textbf{global} \\ \midrule
			FCN  	  & 94.1 & 1.0 & 92.8 & 10.8 & 77 & 77.5 & 58.9 & 93.1\\ \midrule
			P-Net     & 86.9 & 0 & 81.3 & 11.5 & 80 & 56.8     & 52.8 & 85.7\\ \bottomrule
		\end{tabular}%
	%}
	\label{tab:sparse_results}
\end{table*}

\begin{table*}[]
	\centering
	\caption{Evaluation of Knowledge Transference to P-Nets of different sizes.}
	\vspace{-3mm}
	\resizebox{\textwidth}{!}{%
		\scriptsize
		\tabcolsep=0.06cm
		\begin{tabular}{@{}lccccccccccccc@{}}
			\toprule
			Method    & sky & building & road & sidewalk & fence & vegetation & pole & car & sign & pedestrian & cyclist & \textbf{per-class} & \textbf{global} \\ \midrule
			T-Net $\rightarrow$ P-Net 6B (Probs)   & 87.3   	& 75.7     & 87.4   & 28.1      & 9.4     & 83.8    & 6.8    & 89.4   & 24.5    & 55.4         & 6.1      & 50.3                  & 75.3\\ \midrule               

			T-Net $\rightarrow$ P-Net 8B (Probs)       & 85.1   	& 65.1     & 87.5   & 21.1      & 35.7     & 85.3    & 6.6   & 90.0   & 45.2    & 53.2         & 55.6     & 57.3                 & 70.8               \\ \midrule

			T-Net $\rightarrow$ P-Net 10B (Probs)   & 84.1   	& 79.9     & 84.9   & 31.0      & 22.9     & 78.7    & 3.1    & 88.6   & 31.0    & 51.6         & 15.3      & 51.9                 & 75.7 \\ \midrule              
			\midrule
			T-Net $\rightarrow$ P-Net 6B (Probs-drop)   & 87.3   	& 75.7     & 87.4   & 28.1      & 9.4     & 83.8    & 6.8    & 89.4   & 24.5    & 55.4         & 6.1      & 50.3                  & 75.3\\ \midrule               

			T-Net $\rightarrow$ P-Net 8B (Probs-drop)   & 87.6   	& 75.9     & 79.3   & 43.2      & 27.1     & 80.8    & 4.0    & 86.9   & 19.9    & 68.5         & 14.0      & 53.4                  & 74.8\\ \midrule            

			T-Net $\rightarrow$ P-Net 10B (Probs-drop)   & 84.1   	& 79.9     & 84.9   & 31.0      & 22.9     & 78.7    & 3.1    & 88.6   & 31.0    & 51.6         & 15.3      & 51.9                 & 75.7 \\ \midrule              

		\end{tabular}%
	}
	\label{tab:multiblock}
\end{table*}
